Decentralized Federated Averaging

Federated averaging (FedAvg) is a communication efficient algorithm for the distributed training with an enormous number of clients. In FedAvg, clients keep their data locally for privacy protection; a central parameter server is used to communicate between clients. This central server distributes the parameters to each client and collects the updated parameters from clients. FedAvg is mostly studied in centralized fashions, which requires massive communication between server and clients in each communication. Moreover, attacking the central server can break the whole system's privacy. In this paper, we study the decentralized FedAvg with momentum (DFedAvgM), which is implemented on clients that are connected by an undirected graph. In DFedAvgM, all clients perform stochastic gradient descent with momentum and communicate with their neighbors only. To further reduce the communication cost, we also consider the quantized DFedAvgM. We prove convergence of the (quantized) DFedAvgM under trivial assumptions; the convergence rate can be improved when the loss function satisfies the P{\L} property. Finally, we numerically verify the efficacy of DFedAvgM.

==> preamble.tex <==
% ---------------------------------
%floats and figures
% ---------------------------------

% if you need to pass options to natbib, use, e.g.:
\PassOptionsToPackage{numbers, compress}{natbib}
\usepackage{amsmath}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
    citecolor=black
}
\urlstyle{same}
%\usepackage{array}
\usepackage{booktabs} % for professional tables
\usepackage{amsfonts}
\usepackage{bm}
%\usepackage{soul}
%\usepackage{lmodern}
%\usepackage{booktabs}
\usepackage{threeparttable}
%\usepackage{mathtools}
\usepackage{tablefootnote}

%\usepackage{cuted}
\usepackage{lipsum}
\usepackage{comment}

\usepackage{multirow}
%\usepackage[usenames, dvipsnames]{color}
\usepackage{amsmath}

\newcommand\xmod[1]{{\textcolor{blue}{#1}}}
\newcommand\zmod[1]{{\textcolor{red}{#1}}}


\usepackage{hyperref}

\usepackage{enumitem}

\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\usepackage{listings}

\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}

\usepackage{listings}
\usepackage{color}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color
  basicstyle=\footnotesize,        % size of fonts used for the code
  breaklines=true,                 % automatic line breaking only at whitespace
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  keywordstyle=\color{blue},       % keyword style
  stringstyle=\color{mymauve},     % string literal style
}

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}
% \usepackage[disable]{todonotes}
% \usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
%takes in optional argument
% \newcommand{\tocite}[1]{%
% \textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
% }


\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

%version in control in draft mode
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
% \newcommand{\figref}[1]{Fig.    \,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
% \newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

\newcommand{\tss}{\hspace*{0.66mm}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{0.5mm}
\setlength{\belowcaptionskip}{0mm} 
\setlength{\textfloatsep}{1.5mm}
\setlength{\dbltextfloatsep}{1.5mm}
%\renewcommand{\baselinestretch}{.9945}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions for equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

